The cost of fairness in classification

We study the problem of learning classifiers with a fairness constraint, with three main contributions towards the goal of quantifying the problem's inherent tradeoffs. First, we relate two existing fairness measures to cost-sensitive risks. Second, we show that for cost-sensitive classification and fairness measures, the optimal classifier is an instance-dependent thresholding of the class-probability function. Third, we show how the tradeoff between accuracy and fairness is determined by the alignment between the class-probabilities for the target and sensitive features. Underpinning our analysis is a general framework that casts the problem of learning with a fairness requirement as one of minimising the difference of two statistical risks.

==> beyond-classification.tex <==
% !TEX root = fairness-icml17.tex

We now discuss how our analysis may be extended to variants of the fairness-aware problem as posed in Problem \ref{prb:disc-aware}.

%
%\subsection{The constrained fairness problem}
%\label{sec:constrained}

% Our definition of the fairness-aware learning problem (Problem \ref{prb:disc-aware}) was in terms of a linear tradeoff between the performance and fairness measures.
% An alternate setting is a constrained problem:
% for fairness level $\tau \in \Real_+$, find
% \begin{equation}
% 	\label{eqn:fairness-constrained}
% 	f^* \in \argmin{f \in [0, 1]^{\XCal}}{\Perf( f; \D )} \colon \Fairness( f; \DFull ) \geq \tau 
% \end{equation}
% For the case of cost-sensitive performance and fairness measures,
% the objectives in Equations \ref{eqn:fairness-lagrange} and \ref{eqn:fairness-constrained} are related by the Lagrangian principle;
% see Appendix \ref{sec:lagrangian} for more discussion.

% The constrained version of the fairness problem (Equation \ref{eqn:fairness-constrained})
% may be cast as the solution to a simple linear program.
% This is owing to the fact that cost-sensitive risks are linear for randomised classifiers.

% \begin{proposition}
% \label{prop:constrained-opt}
% Pick any distribution $\DFull$ with finite support, costs $c, \bar{c} \in [0, 1]$, and $\tau \in \Real_+$.
% The optimal classifier for %the problem
% $$ \min_{\randClassifier} \CSERR( f; \D, c ) \colon \CSERR^\diamond( f; \DSens, \bar{c} ) \geq \tau $$
% is expressible as a solution to a linear program.
% \end{proposition}

% % While appealing, one disappointing aspect of the above is the lack of any analytic form for the solution.
% % This makes it hard to reason about how precisely the fairness constraint affects the optimal solution.
% %We now see that the unconstrained setting fares better in this regard.

% %In the constrained case,
% The linear program in Proposition \ref{prop:constrained-opt} may be set-up easily for a given problem. %meaning that it is trivial to compute the optimal constrained solution for a range of fairness measures.
% There is however a subtlety:
% in practice, one typically works with a parametric family $\FCal \subseteq [0, 1]^{\XCal}$.
% Here, the resulting optimisation may be non-convex, \eg if one uses randomised classifiers derived from scorers through some nonlinear transform $f = \Psi \circ s$.


%Beyond classification: fairness of class-probability estimators
\subsection{From classifiers to scorers}

% In the class-probability estimation problem,
% our goal is to produce a scorer $\scorer$ that is an monotone transformation of $\eta$.
% Formally, for \emph{loss function} $\ell \colon \Labels \times \Real \to \Real_+$, let the $\ell$-risk be
% \begin{equation}
% 	\label{eqn:cpe-perf}
% 	\CPEPerf( s; \D, \ell ) \defEq \E{(\X, \Y) \sim \D}{ \ell( \Y, s( \X ) ) }.
% \end{equation}
% In class-probability estimation, we work with losses
% %whose Bayes-optimal scorer is
% for which
% $\Psi \circ \eta \in \operatorname{Argmin}_s { \CPEPerf( s; \D, \ell ) }$
% for some monotone $\Psi \colon (0, 1) \to \Real$.
% Such $\ell$ are called \emph{proper composite} with \emph{link function} $\Psi$ \citep{Reid:2010}.
% Examples include the logistic loss $\ell(y,v) = \log(1+e^{-yv})$ with
% %$\Psi( u ) = \log u/(1 - u)$,
% $\Psi(u) = \log \frac{u}{1-u}$,
% and
% exponential loss $\ell(y,v) = e^{-yv}$ with
% %$\Psi(u) = \half \cdot \log u/(1 - u)$.
% $\Psi(u) = \half \cdot \log \frac{u}{1-u}$.

One value of viewing existing fairness measures as particular instances of statistical risks is that we can plug in a broader class of such risks.
For example, for a scorer $\scorer$, we can consider a fairness measure
%(c.f.\ Equation \ref{eqn:cpe-perf})
%$$ \Fairness_{\mathrm{cpe}}( s; \DSens ) = \CPEPerf( s; \DSens, \ell ) $$
$$ \Fairness( s; \DSens ) = \E{(\X, \Y) \sim \D}{ \ell( \Y, s( \X ) ) } $$
for suitable surrogate loss $\ell \colon \Labels \times \Real \to \Real_+$.
Notions of perfect fairness for scorers have been proposed in \citet{Kleinberg:2016}.

...Ratio of weight functions?...

